Optimizing Modular Robot Composition: A Lexicographic Genetic Algorithm Approach

Industrial robots are designed as general-purpose hardware with limited ability to adapt to changing task requirements or environments. Modular robots, on the other hand, offer flexibility and can be easily customized to suit diverse needs. The morphology, i.e., the form and structure of a robot, significantly impacts the primary performance metrics acquisition cost, cycle time, and energy efficiency. However, identifying an optimal module composition for a specific task remains an open problem, presenting a substantial hurdle in developing task-tailored modular robots. Previous approaches either lack adequate exploration of the design space or the possibility to adapt to complex tasks. We propose combining a genetic algorithm with a lexicographic evaluation of solution candidates to overcome this problem and navigate search spaces exceeding those in prior work by magnitudes in the number of possible compositions. We demonstrate that our approach outperforms a state-of-the-art baseline and is able to synthesize modular robots for industrial tasks in cluttered environments.

==> results_table_new.tex <==
\begin{tabular}{lccccc}
\toprule
 &  & Achieved & $C_T$ & $n_J$ & $t_{max}$ \\
\midrule
% \multirow{3}{*}{Synthetic I} & $d = 3$ & 16 & 11.86 & 6.2 & 3.1s \\
%  & $d = 4$ & 10 & 15.16 & 6.8 & 5.7s \\
%  & $d = 5$ & 10 & 16.42 & 6.7 & 7.1s \\
% \cmidrule{1-6}
% \multirow{3}{*}{Synthetic II} & $d = 3$ & 20 & 12.27 & 6.4 & 3.3s \\
%  & $d = 4$ & 20 & 13.80 & 6.7 & 4.6s \\
%  & $d = 5$ & 20 & 15.33 & 6.8 & 5.9s \\
%\cmidrule{1-6}
% \toprule
%\cmidrule{1-6} \\[-12pt]
%\cmidrule{1-6}
\multirow{3}{*}{Manufacturing I} & $t_{o, 1}$ & 10 & 12.81 & 5.3 & 5.0s \\
 & $t_{o, 2}$ & 10 & 14.33 & 6.7 & 5.0s \\
 & $t_{o, 3}$ & 10 & 15.05 & 6.6 & 5.8s \\
\cmidrule{1-6}
\multirow{3}{*}{Manufacturing II} & $t_{o, 1}$ & 10 & 10.15 & 4.5 & 3.4s \\
 & $t_{o, 2}$ & 10 & 12.48 & 6.4 & 3.6s \\
 & $t_{o, 3}$ & 10 & 12.27 & 6.0 & 3.8s \\
% \cmidrule{1-6}
\toprule
\multicolumn{2}{l}{Ours  (Manufacturing)}  & \textbf{10} & \textbf{12.85} & \textbf{5.9} & \textbf{4.5s} \\
\cmidrule{1-6}
Baseline (Manufacturing) &  & 9.8 & 20.06 & 7.5 & 15.0s \\
\cmidrule{1-6} \\[-12pt]
\cmidrule{1-6}
\multicolumn{2}{l}{Ours  (Synthetic)}  & \textbf{16} & \textbf{14.14} & \textbf{6.6} & \textbf{5.0s} \\
\cmidrule{1-6}
Baseline (Synthetic) &  & 15.2 & 19.67 & 8.1 & 15.2s \\
\bottomrule \\[-8pt]
\multicolumn{6}{l}{\scriptsize $C_T$: Cost as defined in eq.~\eqref{eq:task_cost_function}, $n_J$: Number of joints, $t_{max}$: Cycle time}
\end{tabular}

==> todo.tex <==
- New references:
    Matthews2023, Efficient automatic design of robots
    Romiti2023, An Optimization Study on Modular Reconfigurable Robots: Finding the Task-Optimal Design

Based on Reviewer Comments:
- Rename the "synthetic" tasks or explain the meaning in table 1
- Indicate why numbers are bold in table 1
x- Explain tolerance: Why is t not unit norm, why is a single axis enough
x- Is the lexicographic approach a search space pruning? Answer this
- Why did we weight the cost function the way we did?
- What happens if cost function weighting is changed?
- Is the comparison to the baseline fair? After all, baseline optimizes for other things. Compare directly to work done by Esra.
--> Could replace robot mass M by njoints
--> They do not directly optimize for cycle time, because they can't. Equally, they can't do that for "success rate". Still, they perform their own comparison over success rate - and they can't do cycle time.
x- Do the authors think there could be other ways to make the algorithm more efficient? For example, storing previously visited configurations might avoid the evaluation of previously discarded configurations. --> mention the caching


Reviewer 1:
This is with the use of
language with Table 1. I suggest to please define what you
mean by "synthetic" or suggest changing the word synthetic
for something else. While an astute individual will read
the whole paper, most seem to skim over papers and focus on
the tables and images in the course of their research. This
is not a criticism of your work, but the general trend of
researchers taking an abstract, introduction, conclusion
approach to reading the stack of papers that come our way
every day.

The second minor issue is the use of bold for your entry in
the table, is it not the preferred approach to bold the
values that are the lowest regardless of the approach, then
this can be further explained in the discussion section?

I look forward to how this GA approach leads to the
development of hardware? Could a next step be to assemble
the robot based on the chosen components and do a task?

Reviewer 2:
In the definition of the orientation tolerance (page 3,
between equations 1 and 2), why is the vector t not unit
norm? I am also not sure I understand why the orientation
tolerance is defined just by one axis and one angle. Should
it be defined by two degrees of freedom, as in spherical
coordinates?

To my understanding, the lexicographic approach is a way to
reduce the amount of times the algorithm has to compute a
trajectory for the task. This is done by enforcing some
priors (related to feasibility considerations) on the
solutions. Is this not ultimately a way to reduce the
search space, like previous approaches did? If not, why is
it different?

could you elaborate more on the choice of the cost function
(eq 15)? why are the different terms weighted in that way?
why is 1.2s of cycle time equally valuable as creating a
manipulator with one joint less?

how sensitive to the weights in the cost function is the
algorithm? Do you find very different solutions by varying
the contribution of the number of joints and modules versus
the task execution time (for example, if 2s instead of 1.2s
was equally valuable to 1 joint less)?

my understanding is that the baseline is taken from a
previous paper from the same group, and modified slightly.
The results from the baseline algorithm and the one
proposed are compared. The comparison is done over the cost
Ct, the number of joints and the overall task execution
time. However, these three quantities chosen for the
comparison are not at all optimized for in the baseline
approach. Therefore, it is probably not very surprising
that the proposed algorithm outperforms the baseline. I
would suggest the author to extend the comparison to
consider quantities that are optimized by both approaches.
In reference 7 there are multiple interesting objectives
that could be used as comparison metrics.

A genetic algorithm ultimately represents a sampling method
over the design search space. Therefore, in general, it is
computationally expensive. By using a lexicographic
approach, bad solutions are discarded immediately without
proceeding to the evaluation of performances on the task,
and this speeds up the optimization. Do the authors think
there could be other ways to make the algorithm more
efficient? For example, storing previously visited
configurations might avoid the evaluation of previously
discarded configurations.

I would recommend reading the following reference. The
authors adopt a similar approach for design optimization of
legged robots. Perhaps it could offer an insight on some
other approaches for design space exploration.
Zhao, Allan, et al. "Robogrammar: graph grammar for
terrain-optimized robot design." ACM Transactions on
Graphics (TOG) 39.6 (2020): 1-16.
